Gemini-LIGHTS: Herbig Ae/Be and massive T-Tauri protoplanetary disks imaged with Gemini Planet Imager

We present the complete sample of protoplanetary disks from the Gemini- Large Imaging with GPI Herbig/T-tauri Survey (Gemini-LIGHTS) which observed bright Herbig Ae/Be stars and T-Tauri stars in near-infrared polarized light to search for signatures of disk evolution and ongoing planet formation. The 44 targets were chosen based on their near- and mid-infrared colors, with roughly equal numbers of transitional, pre-transitional, and full disks. Our approach explicitly did not favor well-known, "famous" disks or those observed by ALMA, resulting in a less-biased sample suitable to probe the major stages of disk evolution during planet formation. Our optimized data reduction allowed polarized flux as low as 0.002% of the stellar light to be detected, and we report polarized scattered light around 80% of our targets. We detected point-like companions for 47% of the targets, including 3 brown dwarfs (2 confirmed, 1 new), and a new super-Jupiter mass candidate around V1295 Aql. We searched for correlations between the polarized flux and system parameters, finding a few clear trends: presence of a companion drastically reduces the polarized flux levels, far-IR excess correlates with polarized flux for non-binary systems, and systems hosting disks with ring structures have stellar masses $<$ 3 Msun. Our sample also included four hot, dusty "FS CMa" systems and we detected large-scale ($>100$ au) scattered light around each, signs of extreme youth for these enigmatic systems. Science-ready images are publicly available through multiple distribution channels using a new FITS file standard jointly developed with members of the VLT/SPHERE team.

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/companion_results_publish_latex.tex <==
\clearpage
%\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{lcccccccc}
\tablecaption{Point Sources Detected in Gemini-LIGHTS sample}
\small
\tablehead{
\colhead{Target} & \colhead{Band} & \colhead{Epoch} & \colhead{Comp. \#} & \colhead{Separation} & \colhead{PA} & \colhead{Flux} & \colhead{Saturated} & \colhead{Mass Est.} \\
\colhead{} & \colhead{} & \colhead{(YYYYMMDD)} & \colhead{}  & \colhead{(``)} & \colhead{($^{\circ}$)} & \colhead{(mJy)} & \colhead{} & \colhead{(\Msun)}}
\label{tbl:companion_results}
\startdata
FU Ori & J & 20180103 & 1 & 0.431 $\pm$ 0.003 & 163.3 $\pm$ 0.3 & 27 $\pm$ 4 & TRUE & 0.6 $_{-0.1} ^{+0.1}$ \\ 
HD 100453 & J & 20150411 & 1 & 0.909 $\pm$ 0.002 & 131.63 $\pm$ 0.09 & 15.4 $\pm$ 1.3 & FALSE & 0.08 $_{-0.04} ^{+0.01}$ \\ 
HD 101412 & H & 20180319 & 1 & 0.460 $\pm$ 0.002 & 149.9 $\pm$ 0.2 & 1.46 $\pm$ 0.11 & FALSE & 0.053 $_{-0.003} ^{+0.03}$ \\ 
HD 101412 & H & 20180319 & 2 & 0.153 $\pm$ 0.003 & 184.9 $\pm$ 1.0 & 5.0 $\pm$ 0.4 & FALSE & 0.19 $_{-0.01} ^{+0.06}$ \\ 
HD 104237 & J & 20170407 & 1 & 1.226 $\pm$ 0.004 & 255.43 $\pm$ 0.14 & 29 $\pm$ 9 & FALSE & 0.11 $_{-0.04} ^{+0.04}$ \\ 
HD 104237 & J & 20180317 & 1 & 1.214 $\pm$ 0.004 & 255.034 $\pm$ 0.13 & 19 $\pm$ 6 & FALSE & 0.065 $_{-0.02} ^{+0.02}$ \\ 
HD 104237 & J & 20180520 & 1 & 1.204 $\pm$ 0.003 & 255.1 $\pm$ 0.11 & 32 $\pm$ 6 & FALSE & 0.12 $_{-0.02} ^{+0.02}$ \\ 
HD 104237 & J & 20190217 & 1 & 1.198 $\pm$ 0.004 & 255.28 $\pm$ 0.11 & 34 $\pm$ 5 & FALSE & 0.13 $_{-0.02} ^{+0.02}$ \\ 
HD 144432 & H & 20150708 & 1 & 1.256 $\pm$ 0.004 & 6.07 $\pm$ 0.16 & 51 $\pm$ 7 & TRUE & 0.3 $_{-0.05} ^{+0.03}$ \\ 
HD 158643 & J & 20180609 & 1 & 0.118 $\pm$ 0.013 & 294 $\pm$ 5 & 30 $\pm$ 4 & FALSE & 0.07 $_{-0.02} ^{+0.01}$ \\ 
HD 38087 & J & 20180103 & 1 & 0.303 $\pm$ 0.003 & 183.7 $\pm$ 0.4 & 47 $\pm$ 8 & TRUE & 0.8 $_{-0.3} ^{+0.5}$ \\ 
HD 50138 & J & 20180104 & 1 & 0.729 $\pm$ 0.003 & 106.6 $\pm$ 0.2 & 10.1 $\pm$ 1.5 & FALSE & $^\ast$0.12    \\ 
HD 98800 & H & 20190127 & 1 & 0.374 $\pm$ 0.010 & 9.8 $\pm$ 0.6 & 633 $\pm$ 9 & TRUE & 0.4 $_{-0.03} ^{+0.03}$ \\ 
HR 5999 & J & 20170406 & 1 & 1.251 $\pm$ 0.004 & 112.55 $\pm$ 0.11 & 141 $\pm$ 16 & TRUE & 0.6 $_{-0.2} ^{+0.1}$ \\ 
HR 5999 & J & 20170702 & 1 & 1.260 $\pm$ 0.005 & 112.4 $\pm$ 0.2 & 128 $\pm$ 19 & TRUE & 0.6 $_{-0.2} ^{+0.1}$ \\ 
HT Lup & H & 20190514 & 1 & 0.161 $\pm$ 0.003 & 246.6 $\pm$ 0.7 & 70 $\pm$ 7 & TRUE & 0.13 $_{-0.01} ^{+0.01}$ \\ 
Hen 3-365 & J & 20170406 & 1 & 0.818 $\pm$ 0.003 & 101.08 $\pm$ 0.14 & 1.3 $\pm$ 0.2 & FALSE & $^\ast$0.17    \\ 
Hen 3-365 & J & 20170406 & 2 & 0.446 $\pm$ 0.008 & 133.0 $\pm$ 0.8 & 0.6 $\pm$ 0.1 & FALSE & $^\ast$0.13    \\ 
Hen 3-225 & J & 20190127 & 1 & 1.564 $\pm$ 0.019 & 303.4 $\pm$ 0.3 & 1.46 $\pm$ 0.02 & FALSE & $^\ast$0.12    \\ 
Hen 3-1330 & J & 20190512 & 1 & 0.268 $\pm$ 0.017 & 49 $\pm$ 2 & 0.8 $\pm$ 0.3 & FALSE & $^\ast$0.13    \\ 
MWC 147 & J & 20171231 & 1 & 0.137 $\pm$ 0.004 & 56 $\pm$ 1 & 30 $\pm$ 6 & TRUE & 0.6 $_{-0.1} ^{+0.4}$ \\ 
MWC 147 & J & 20190127 & 1 & 0.156 $\pm$ 0.003 & 54.1 $\pm$ 0.8 & 33 $\pm$ 5 & TRUE & 0.5 $_{-0.1} ^{+0.4}$ \\ 
MWC 166 & J & 20170406 & 1 & 0.587 $\pm$ 0.004 & 298.4 $\pm$ 0.3 & 282 $\pm$ 9 & TRUE & $^\ast >$1.4    \\ 
MWC 297 & H & 20180608 & 1 & 0.573 $\pm$ 0.003 & 86.5 $\pm$ 0.2 & 2.06 $\pm$ 0.09 & FALSE & $^\ast$0.04    \\ 
MWC 297 & H & 20180817 & 1 & 0.576 $\pm$ 0.004 & 86.6 $\pm$ 0.2 & 1.74 $\pm$ 0.14 & FALSE & $^\ast$0.04    \\ 
MWC 789 & H & 20181120 & 1 & 0.371 $\pm$ 0.002 & 216.8 $\pm$ 0.3 & 10.7 $\pm$ 0.8 & FALSE & 0.8 $_{-0.2} ^{+0.1}$ \\ 
MWC 863 & J & 20140421 & 1 & 0.975 $\pm$ 0.004 & 226.97 $\pm$ 0.14 & 154 $\pm$ 19 & TRUE & 0.8 $_{-0.1} ^{+0.1}$ \\ 
Ty CrA & H & 20180608 & 1 & 0.129 $\pm$ 0.004 & 255.2 $\pm$ 1.3 & 26 $\pm$ 4 & FALSE & $>$1.4    \\ 
Ty CrA & H & 20180817 & 1 & 0.112 $\pm$ 0.003 & 257.3 $\pm$ 1.0 & 41 $\pm$ 4 & FALSE & $>$1.4    \\ 
V921 Sco & H & 20190513 & 1 & 0.475 $\pm$ 0.013 & 319.0 $\pm$ 1.1 & 0.09 $\pm$ 0.03 & FALSE & 0.03 $_{-0.01} ^{+0.01}$ \\ 
V921 Sco & H & 20190513 & 2 & 1.122 $\pm$ 0.003 & 323.12 $\pm$ 0.09 & 0.96 $\pm$ 0.08 & FALSE & 0.15 $_{-0.01} ^{+0.01}$ \\ 
V1295 Aql & H & 20180608 & 1 & 1.113 $\pm$ 0.003 & 40.52 $\pm$ 0.11 & 0.026 $\pm$ 0.002 & FALSE & $^\ast $0.010    \\ 
V1295 Aql & H & 20180816 & 1 & 1.135 $\pm$ 0.016 & 40.1 $\pm$ 0.5 & 0.055 $\pm$ 0.009 & FALSE & $^\ast $0.013    \\ 
V1295 Aql & J & 20180817 & 1 & 1.119 $\pm$ 0.005 & 40.6 $\pm$ 0.2 & 0.015 $\pm$ 0.002 & FALSE & $^\ast $0.010    \\ 
\enddata
\tablecomments{Point sources with their PSF cores saturated are noted in the table. Mass estimate based on measured companion flux and the system age (see Table \ref{tbl:target_properties}). Mass estimates use models from \citet{Baraffe2015} for masses $>$ 0.01 \Msun{} and \citet{Phillips2020} for masses $<$ 0.01 \Msun{}. A $\ast $ denotes any target with ages $<$ 0.5 Myr which are younger than the youngest model in \citet{Baraffe2015} or \citet{Phillips2020}.}
\end{deluxetable*}
%\end{longrotatetable}

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/epochs_parameters_publish.tex <==
\clearpage
%\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{lccccc}
\tablecaption{Polarization Flux and Point Source Detection Upper Limits}
\small
\tablehead{
\colhead{Target} & \colhead{Band} & \colhead{Epoch} & \colhead{\Qphi/Fstar}  & \multicolumn{2}{c}{5$\sigma$ Point Source Detection Upper limit} \\
\colhead{} & \colhead{} & \colhead{(YYYYMMDD)} & \colhead{(per 1000)} & \colhead{Contrast at 0$\farcs$2} & \colhead{Mass Sensitivity (\Msun)}}
\startdata
AK Sco & H & 20180811 & 1.2 $\pm$ 0.2 & 1.6E-04 & 0.011  \\ 
CU Cha & J & 20170406 & 2.7 $\pm$ 0.9 & 3.9E-05 & 0.006  \\ 
CU Cha & H & 20180413 & 3.8 $\pm$ 1.0 & 2.5E-04 & 0.02  \\ 
FU Ori & J & 20180103 & 3.7 $\pm$ 0.6 & 1.2E-04 & 0.03  \\ 
GW Ori & J & 20180104 & 9.4 $\pm$ 0.9 & 1.6E-04 & 0.011  \\ 
GW Ori & H & 20180104 & 13.3 $\pm$ 1.1 & 5.9E-05 & 0.007  \\ 
HD 34700 A & J & 20180103 & 15.7 $\pm$ 1.8 & 1.3E-04 & 0.008  \\ 
HD 34700 A & H & 20180103 & 22.2 $\pm$ 1.8 & 5.3E-05 & 0.005  \\ 
HD 36917 & J & 20171231 & $<$0.02 &  3.6E-05 & 0.007  \\ 
HD 36917 & H & 20190126 & $<$0.03 &  8.6E-05 & 0.01  \\ 
HD 37806 & J & 20171231 & $<$0.04 &  3.8E-05 & 0.008  \\ 
HD 38087 & J & 20180103 & $<$0.12 &  6.1E-05 & 0.008  \\ 
HD 45677 & J & 20171231 & 8.4 $\pm$ 1.1 & 5.5E-05 & 0.01  \\ 
HD 45677 & H & 20180101 & 6.9 $\pm$ 1.0 & 3.0E-05 & 0.01  \\ 
HD 50138 & J & 20180104 & 0.9 $\pm$ 0.2 & 6.0E-05 & 0.011  \\ 
HD 85567 & J & 20180103 & 0.10 $\pm$ 0.08 & 1.0E-04 & 0.03  \\ 
HD 85567 & J & 20180520 & 0.12 $\pm$ 0.07 & 4.7E-05 & 0.02  \\ 
HD 85567 & H & 20190127 & 0.13 $\pm$ 0.11 & 2.5E-04 & 0.06  \\ 
HD 95881 & J & 20180104 & $<$0.09 &  9.6E-05 & 0.03  \\ 
HD 98800 & H & 20190127 & 0.19 $\pm$ 0.14 & \nodata & \nodata  \\ 
HD 98922 & J & 20180321 & 0.21 $\pm$ 0.16 & 6.9E-05 & 0.03  \\ 
HD 100453 & J & 20150410 & 2.9 $\pm$ 0.2 & \nodata & \nodata  \\ 
HD 100546 & J & 20170220 & 10.2 $\pm$ 0.6 & 8.7E-05 & 0.008  \\ 
HD 101412 & H & 20180319 & $<$0.04 &  1.7E-04 & 0.013  \\ 
HD 104237 & J & 20170407 & 0.04 $\pm$ 0.03 & 9.2E-05 & 0.013  \\ 
HD 104237 & J & 20180317 & 0.03 $\pm$ 0.02 & 1.6E-04 & 0.014  \\ 
HD 104237 & J & 20180520 & 0.06 $\pm$ 0.03 & 2.2E-04 & 0.02  \\ 
HD 104237 & J & 20190217 & $<$0.06 &  1.4E-04 & 0.014  \\ 
HD 139614 & J & 20170406 & 2.5 $\pm$ 0.7 & 8.9E-05 & 0.01  \\ 
HD 139614 & J & 20190513 & 1.5 $\pm$ 0.6 & 6.7E-05 & 0.009  \\ 
HD 139614 & H & 20180608 & 2.5 $\pm$ 0.7 & 3.1E-03 & 0.06  \\ 
HD 141569 & J & 20180609 & 0.29 $\pm$ 0.28 & 1.5E-04 & 0.013  \\ 
HD 141569 & J & 20190223 & $<$0.3 &  4.8E-05 & 0.007  \\ 
HD 142527 & H & 20140425 & 9.26 $\pm$ 1.17 & \nodata & \nodata  \\ 
HD 142666 & J & 20170703 & 0.19 $\pm$ 0.17 & \nodata & \nodata  \\ 
HD 142666 & J & 20180609 & 0.09 $\pm$ 0.08 & \nodata & \nodata  \\ 
HD 144432 & H & 20150709 & $<$0.03 &  \nodata & \nodata  \\ 
HD 145718 & J & 20180607 & 0.4 $\pm$ 0.3 & 4.4E-05 & 0.007  \\ 
HD 145718 & H & 20180608 & 0.4 $\pm$ 0.2 & 1.1E-04 & 0.011  \\ 
HD 158643 & J & 20180609 & $<$0.01 &  2.4E-05 & 0.005  \\ 
HD 158643 & J & 20190223 & $<$0.04 &  \nodata & \nodata  \\ 
HD 169142 & J & 20140425 & 4.5 $\pm$ 0.8 & 1.0E-04 & 0.008  \\ 
HD 176386 & J & 20180817 & $<$0.01 &  2.8E-05 & 0.005  \\ 
HD 176386 & H & 20180607 & $<$0.05 &  6.7E-05 & 0.006  \\ 
HD 176386 & H & 20180816 & $<$0.02 &  6.8E-05 & 0.006  \\ 
Hen 3-1330 & J & 20190512 & $<$0.03 &  4.8E-05 & 0.04  \\ 
Hen 3-225 & J & 20190127 & $<$0.04 &  7.3E-05 & 0.013  \\ 
Hen 3-225 & H & 20190127 & $<$0.06 &  6.7E-05 & 0.01  \\ 
Hen 3-365 & J & 20170406 & 5.5 $\pm$ 0.6 & 3.3E-05 & 0.05  \\ 
HR 5999 & J & 20170406 & $<$0.02 &  3.3E-04 & 0.03  \\ 
HR 5999 & J & 20170702 & 0.03 $\pm$ 0.02 & 7.8E-05 & 0.01  \\ 
HT Lup & H & 20190514 & 0.4 $\pm$ 0.2 & 5.6E-04 & 0.009  \\ 
MWC 147 & J & 20171231 & $<$0.07 &  8.4E-05 & 0.011  \\ 
MWC 147 & H & 20190127 & $<$0.1 &  3.3E-04 & 0.04  \\ 
MWC 166 & J & 20170406 & $<$0.06 &  6.0E-03 & 1.4  \\ 
MWC 275 & J & 20140424 & 0.3 $\pm$ 0.2 & 7.3E-05 & 0.01  \\ 
MWC 297 & H & 20180608 & 0.3 $\pm$ 0.2 & 8.5E-05 & 0.04  \\ 
MWC 297 & H & 20180817 & 0.3 $\pm$ 0.2 & 1.0E-04 & 0.04  \\ 
MWC 614 & J & 20180816 & 2.0 $\pm$ 0.3 & 1.5E-04 & 0.014  \\ 
MWC 614 & H & 20180816 & 2.4 $\pm$ 0.2 & 1.7E-04 & 0.013  \\ 
MWC 789 & H & 20181120 & 5.9 $\pm$ 1.5 & 6.3E-04 & 0.06  \\ 
MWC 863 & J & 20140424 & $<$0.3 &  1.1E-03 & 0.03  \\ 
PDS 66 & J & 20160306 & 2.2 $\pm$ 1.1 & 5.9E-05 & 0.003  \\ 
Ty CrA & H & 20180608 & $<$0.6 &  8.7E-04 & 0.3  \\ 
Ty CrA & H & 20180817 & $<$0.44 &  1.5E-04 & 0.06  \\ 
V1295 Aql & J & 20180816 & $<$0.02 &  2.5E-04 & 0.05  \\ 
V1295 Aql & H & 20180608 & $<$0.02 &  1.0E-04 & 0.03  \\ 
V1295 Aql & H & 20180816 & $<$0.04 &  2.9E-04 & 0.05  \\ 
V921 Sco & H & 20190513 & 0.06 $\pm$ 0.05 & 1.6E-04 & 0.13  \\ 
WRAY 15-535 & J & 20180319 & 0.11 $\pm$ 0.07 & 1.0E-04 & \nodata  \\ 
WRAY 15-535 & J & 20190222 & $<$0.04 &  1.5E-05 & \nodata  \\ 
\enddata
\tablecomments{Mass estimate based on measured companion flux and the system age (see Table \ref{tbl:target_properties} and use models from \citet{Baraffe2015} for masses $>$ 0.01 \Msun{} and \citet{Phillips2020} for masses $<$ 0.01 \Msun{}. \Qphi/Fstar values utilized in this work are the weighted average of the epochs listed above.}\label{tbl:epoch_parameters}
\end{deluxetable*}

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/target_SED_table.tex <==
\startlongtable
\begin{deluxetable*}{lccccc}
\tablecaption{Gemini-LIGHTS Photometry and Meeus Group}
\tablehead{
\colhead{Target} & \colhead{WISE 2} & \colhead{WISE 4} & \colhead{J-band} & \colhead{H-band} & \colhead{Meeus Group} \\
\colhead{} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{}}
\label{tbl:target_SED_table}
\startdata
AK Sco & 4.8$\pm$ 0.036 & 0.888$\pm$ 0.023 & 7.676$\pm$ 0.026 & 7.059$\pm$ 0.033 & II  \\ 
CU Cha & 4.3$\pm$ 0.043 & -1.309$\pm$ 0.013 & 7.267$\pm$ 0.023 & 6.665$\pm$ 0.049 & I  \\ 
FU Ori & 3.509$\pm$ 0.065 & 0.175$\pm$ 0.021 & 6.519$\pm$ 0.023 & 5.699$\pm$ 0.033 & \nodata   \\ 
GW Ori & 4.208$\pm$ 0.045 & -0.74$\pm$ 0.011 & 7.698$\pm$ 0.03 & 7.103$\pm$ 0.029 & I  \\ 
HD 100453 & 3.388$\pm$ 0.065 & -1.355$\pm$ 0.007 & 6.945$\pm$ 0.026 & 6.39$\pm$ 0.038 & I  \\ 
HD 100546 & 3.156$\pm$ 0.049 & -3.565$\pm$ 0.001 & 6.425$\pm$ 0.02 & 5.962$\pm$ 0.031 & I  \\ 
HD 101412 & 4.94$\pm$ 0.031 & 1.325$\pm$ 0.013 & 8.635$\pm$ 0.023 & 8.217$\pm$ 0.047 & II  \\ 
HD 104237 & 2.469$\pm$ 0.071 & -0.909$\pm$ 0.009 & 5.813$\pm$ 0.023 & 5.246$\pm$ 0.059 & II  \\ 
HD 139614 & 5.099$\pm$ 0.03 & -0.667$\pm$ 0.008 & 7.669$\pm$ 0.026 & 7.333$\pm$ 0.04 & I  \\ 
HD 141569 & 6.469$\pm$ 0.02 & 1.847$\pm$ 0.012 & 6.872$\pm$ 0.027 & 6.861$\pm$ 0.04 & I  \\ 
HD 142527 & 3.066$\pm$ 0.076 & -0.794$\pm$ 0.009 & 6.503$\pm$ 0.029 & 5.715$\pm$ 0.031 & II  \\ 
HD 142666 & 4.145$\pm$ 0.049 & -0.065$\pm$ 0.023 & 7.351$\pm$ 0.026 & 6.739$\pm$ 0.027 & II  \\ 
HD 144432 & 4.398$\pm$ 0.044 & 0.042$\pm$ 0.016 & 7.095$\pm$ 0.032 & 6.538$\pm$ 0.067 & II  \\ 
HD 145718 & 4.848$\pm$ 0.04 & 0.585$\pm$ 0.015 & 7.69$\pm$ 0.024 & 7.263$\pm$ 0.029 & II  \\ 
HD 158643 & 2.171$\pm$ 0.091 & -0.028$\pm$ 0.014 & 4.9$\pm$ 0.186 & 4.712$\pm$ 0.206 & II  \\ 
HD 169142 & 5.593$\pm$ 0.023 & -0.561$\pm$ 0.008 & 7.31$\pm$ 0.021 & 6.911$\pm$ 0.038 & I  \\ 
HD 176386 & 6.074$\pm$ 0.015 & -0.455$\pm$ 0.012 & 6.847$\pm$ 0.02 & 6.809$\pm$ 0.031 & I  \\ 
HD 34700 A & 6.794$\pm$ 0.016 & 0.993$\pm$ 0.008 & 8.041$\pm$ 0.023 & 7.706$\pm$ 0.023 & I  \\ 
HD 36917 & 4.278$\pm$ 0.044 & 1.153$\pm$ 0.025 & 7.221$\pm$ 0.019 & 6.964$\pm$ 0.034 & II  \\ 
HD 37806 & 3.419$\pm$ 0.115 & 0.116$\pm$ 0.051 & 7.115$\pm$ 0.02 & 6.252$\pm$ 0.033 & II  \\ 
HD 38087 & 7.207$\pm$ 0.018 & 1.889$\pm$ 0.019 & 7.588$\pm$ 0.024 & 7.386$\pm$ 0.042 & I  \\ 
HD 45677 & 1.812$\pm$ 0.03 & -2.895$\pm$ 0.001 & 7.242$\pm$ 0.026 & 6.347$\pm$ 0.023 & I  \\ 
HD 50138 & 1.585$\pm$ 0.08 & -2.078$\pm$ 0.001 & 5.856$\pm$ 0.027 & 5.093$\pm$ 0.029 & II  \\ 
HD 85567 & 3.291$\pm$ 0.062 & 0.454$\pm$ 0.016 & 7.472$\pm$ 0.024 & 6.68$\pm$ 0.031 & II  \\ 
HD 95881 & 3.125$\pm$ 0.069 & 0.513$\pm$ 0.008 & 7.384$\pm$ 0.026 & 6.662$\pm$ 0.044 & II  \\ 
HD 98800 & 5.325$\pm$ 0.032 & 0.194$\pm$ 0.01 & 6.397$\pm$ 0.02 & 5.759$\pm$ 0.027 & \nodata   \\ 
HD 98922 & 1.863$\pm$ 0.014 & -1.054$\pm$ 0.006 & 6.004$\pm$ 0.02 & 5.226$\pm$ 0.029 & II  \\ 
Hen 3-1330 & 3.344$\pm$ 0.063 & 1.95$\pm$ 0.02 & 6.713$\pm$ 0.024 & 6.103$\pm$ 0.042 & \nodata   \\ 
Hen 3-225 & 7.066$\pm$ 0.02 & 4.193$\pm$ 0.027 & 7.818$\pm$ 0.024 & 7.858$\pm$ 0.04 & II  \\ 
Hen 3-365 & 2.248$\pm$ 0.018 & -3.988$\pm$ 0.001 & 6.217$\pm$ 0.037 & 4.756$\pm$ 0.268 & \nodata   \\ 
HR 5999 & 1.895$\pm$ 0.012 & -0.541$\pm$ 0.01 & 5.907$\pm$ 0.018 & 5.22$\pm$ 0.027 & II  \\ 
HT Lup & 4.973$\pm$ 0.032 & 0.856$\pm$ 0.016 & 7.573$\pm$ 0.021 & 6.866$\pm$ 0.029 & \nodata   \\ 
MWC 147 & 3.169$\pm$ 0.074 & -0.757$\pm$ 0.013 & 7.454$\pm$ 0.026 & 6.666$\pm$ 0.034 & II  \\ 
MWC 166 & 4.538$\pm$ 0.044 & 1.051$\pm$ 0.059 & 6.332$\pm$ 0.02 & 6.22$\pm$ 0.033 & \nodata   \\ 
MWC 275 & 2.466$\pm$ 0.061 & -0.758$\pm$ 0.007 & 6.195$\pm$ 0.021 & 5.531$\pm$ 0.036 & II  \\ 
MWC 297 & 1.872$\pm$ 0.018 & -4.718$\pm$ 0.001 & 6.127$\pm$ 0.019 & 4.387$\pm$ 0.214 & \nodata   \\ 
MWC 614 & 3.647$\pm$ 0.051 & -1.606$\pm$ 0.006 & 6.994$\pm$ 0.02 & 6.645$\pm$ 0.026 & I  \\ 
MWC 789 & 4.633$\pm$ 0.039 & 0.046$\pm$ 0.015 & 8.475$\pm$ 0.02 & 7.528$\pm$ 0.026 & II  \\ 
MWC 863 & 3.244$\pm$ 0.065 & -0.592$\pm$ 0.012 & 6.947$\pm$ 0.02 & 6.214$\pm$ 0.02 & II  \\ 
PDS 66 & 6.183$\pm$ 0.022 & 1.587$\pm$ 0.016 & 8.277$\pm$ 0.032 & 7.641$\pm$ 0.023 & \nodata   \\ 
Ty CrA & 5.139$\pm$ 0.027 & -2.35$\pm$ 0.011 & 7.486$\pm$ 0.024 & 6.97$\pm$ 0.026 & I  \\ 
V1295 Aql & 3.443$\pm$ 0.064 & 0.589$\pm$ 0.016 & 7.194$\pm$ 0.019 & 6.647$\pm$ 0.017 & II  \\ 
V921 Sco & 2.045$\pm$ 0.02 & -4.143$\pm$ 0.001 & 7.235$\pm$ 0.027 & 5.918$\pm$ 0.045 & \nodata   \\ 
WRAY 15-535 & 1.556$\pm$ 0.011 & -0.231$\pm$ 0.011 & 5.762$\pm$ 0.018 & 4.959$\pm$ 0.059 & \nodata   \\ 
\enddata
\tablecomments{WISE photometry from WISE ALL-SKY survey \citep{Cutri2012} and J- and H-band photometry from 2MASS survey \citep{Cutri2003}. Meeus Group categorized in this work as described in section \ref{sec:trends}. Notes: (a) \citep{Lieman2016}, (b)	\citep{Henning1993}, (c) \citep{Liu2018}, (d) \citep{Fang2017}, (e)	This Work, (f) \citep{Sylvester1996}, (g) \citep{Plas2019}, (h) \citep{Miley2019}, (i) \citep{Nilsson2010}, (j) \citep{Kataoka2016}, (k) \citep{Ansdell2018}, (l) \citep{Andrews2018}, (m) \citep{Cazzoletti2019}, (n) \citep{Benac2020}}
\end{deluxetable*}

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/target_coords.tex <==
\clearpage
%\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{lccccc}
\tablecaption{Gemini-LIGHTS Target Sample}
\small
\tablehead{
\colhead{Target} & \colhead{HD Name} & \colhead{2MASS Name} & \colhead{RA} & \colhead{Dec} & \colhead{Distance} \\
\colhead{} & \colhead{} & \colhead{} & \colhead{($^{\circ}$)} & \colhead{Dec ($^{\circ}$)} & \colhead{(pc)}}
\label{tbl:target_coords}
\startdata
AK Sco & HD 152404 & 16544485-3653185 & 253.6868708 & -36.8887086 & 139.8$\pm$ 0.6  \\ 
CU Cha & HD 97048 & 11080329-7739174 & 167.013825 & -77.6548583 & 184.4$\pm$ 0.8  \\ 
FU Ori & \nodata & 05452235+0904123 & 86.3431986 & 9.0700691 & 407.5$\pm$ 3.0  \\ 
GW Ori & HD 244138 & 05290838+1152126 & 82.2849625 & 11.8701944 & 408.0$\pm$ 10.4  \\ 
HD 34700 A & HD 34700 & 05194140+0538428 & 79.9225333 & 5.6452111 & 350.5$\pm$ 2.5  \\ 
HD 36917 & HD 36917 & 05344698-0534145 & 83.6957719 & -5.5707229 & 450.4$\pm$ 11.3  \\ 
HD 37806 & HD 37806 & 05410229-0243006 & 85.2595665 & -2.7168744 & 401.6$\pm$ 4.4  \\ 
HD 38087 & HD 38087 & 05430057-0218454 & 85.752413 & -2.3125911 & 377.0$\pm$ 5.4  \\ 
HD 45677 & HD 45677 & 06281742-1303109 & 97.0726019 & -13.0530934 & 572.1$\pm$ 14.6  \\ 
HD 50138 & HD 50138 & 06513340-0657592 & 102.8891461 & -6.9664934 & 351.0$\pm$ 5.7  \\ 
HD 85567 & HD 85567 & 09502853-6058029 & 147.6188579 & -60.9674551 & 1047.4$\pm$ 18.0  \\ 
HD 95881 & HD 95881 & 11015764-7130484 & 165.4900393 & -71.5134176 & 1109.9$\pm$ 24.3  \\ 
HD 98800 & HD 98800 & 11220530-2446393 & 170.5215893 & -24.7778864 & 42.1$\pm$ 1.0  \\ 
HD 98922 & HD 98922 & 11223166-5322114 & 170.631975 & -53.3698472 & 650.9$\pm$ 8.8  \\ 
HD 100453 & HD100453 & 11330559-5419285 & 173.2730745 & -54.3246148 & 103.8$\pm$ 0.2  \\ 
HD 100546 & HD100546 & 11332542-7011412 & 173.3558188 & -70.1947875 & 108.1$\pm$ 0.4  \\ 
HD 101412 & HD 101412 & 11394445-6010278 & 174.9352141 & -60.1743876 & 412.2$\pm$ 2.5  \\ 
HD 104237 & HD 104237 & 12000511-7811346 & 180.0211875 & -78.1929333 & 106.6$\pm$ 0.5  \\ 
HD 139614 & HD 139614 & 15404638-4229536 & 235.1931708 & -42.4983306 & 133.6$\pm$ 0.5  \\ 
HD 141569 & HD 141569 & 15495775-0355162 & 237.4905224 & -3.9213039 & 111.6$\pm$ 0.4  \\ 
HD 142527 & HD 142527 & 15564188-4219232 & 239.1744971 & -42.323228 & 159.3$\pm$ 0.7  \\ 
HD 142666 & HD 142666 & 15564002-2201400 & 239.1667625 & -22.0277806 & 146.3$\pm$ 0.5  \\ 
HD 144432 & HD 144432 & 16065795-2743094 & 241.7414345 & -27.7195047 & 154.8$\pm$ 0.6  \\ 
HD 145718 & HD 145718 & 16131158-2229066 & 243.2982588 & -22.4853188 & 154.7$\pm$ 0.5  \\ 
HD 158643 & HD 158643 & 17312497-2357453 & 262.8540017 & -23.9627733 & 125.7$\pm$ 1.7  \\ 
HD 169142 & HD 169142 & 18242978-2946492 & 276.1240709 & -29.7805404 & 114.9$\pm$ 0.4  \\ 
HD 176386 & HD 176386 & 19013892-3653264 & 285.4122394 & -36.890856 & 155.1$\pm$ 0.7  \\ 
Hen 3-1330 & HD 326823 & 17065390-4236397 & 256.7246196 & -42.6110631 & 1445.2$\pm$ 40.0  \\ 
Hen 3-225 & HD 76534 & 08550867-4327596 & 133.7862435 & -43.4666156 & 885.0$\pm$ 23.1  \\ 
Hen 3-365 & HD 87643 & 10043028-5839521 & 151.1265 & -58.6645278 & 1589.1$\pm$ 309.7  \\ 
HR 5999 & HD 144668 & 16083427-3906181 & 242.142875 & -39.1050278 & 158.6$\pm$ 0.9  \\ 
HT Lup & \nodata & 15451286-3417305 & 236.3036208 & -34.2918389 & 153.5$\pm$ 1.3  \\ 
MWC 147 & HD 259431 & 06330519+1019199 & 98.2716174 & 10.3222059 & 653.4$\pm$ 11.6  \\ 
MWC 166 & HD 53367 & 07042551-1027156 & 106.1063792 & -10.4543722 & 1219.6$\pm$ 314.4  \\ 
MWC 275 & HD163296 & 17562128-2157218 & 269.0886685 & -21.9562308 & 101.0$\pm$ 0.4  \\ 
MWC 297 & \nodata & 18273952-0349520 & 276.9146958 & -3.831125 & 417.8$\pm$ 5.3  \\ 
MWC 614 & HD 179218 & 19111124+1547155 & 287.7969193 & 15.7875669 & 260.1$\pm$ 2.2  \\ 
MWC 789 & HD 250550 & 06015998+1630567 & 90.4999527 & 16.5157295 & 760.3$\pm$ 28.5  \\ 
MWC 863 & HD150193 & 16401792-2353452 & 250.0746503 & -23.8959517 & 150.8$\pm$ 0.5  \\ 
PDS 66 & \nodata & 13220753-6938121 & 200.5314458 & -69.6367194 & 97.9$\pm$ 0.1  \\ 
Ty CrA & \nodata & 19014081-3652337 & 285.4201238 & -36.8762242 & 159.1$\pm$ 4.4  \\ 
V1295 Aql & HD 190073 & 20030250+0544166 & 300.7604637 & 5.7379176 & 847.9$\pm$ 22.5  \\ 
V921 Sco & \nodata & 16590677-4242083 & 254.7782539 & -42.7023413 & 1482.4$\pm$ 77.4  \\ 
WRAY 15-535 & \nodata & 10152198-5751427 & 153.841516 & -57.8618381 & 4989.9$\pm$ 478.1  \\ 
\enddata
\tablecomments{ Distances from Gaia DR3 early release  \citet{Gaia2021}.  }
\end{deluxetable*}
%\end{longrotatetable}

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/target_observational_log.tex <==
\startlongtable
\begin{deluxetable*}{lcccccccc}
\tablecaption{Observational Log and Stellar/Instrumental Polarization}
\tablehead{
\colhead{Target} & \colhead{Filter} & \colhead{Epoch} & \colhead{Exposure Time} & \colhead{\# of Frames} & \multicolumn{2}{c}{Stellar/Instrumental Polarization} \\
\colhead{} & \colhead{} & \colhead{(YYYYMMDD)} & \colhead{(s)} & \colhead{} & \colhead{\% Pol} & \colhead{PA ($^\circ$)}}
\label{tbl:obs_log}
\startdata
AK Sco & H & 20180811 & 59.6 & 40 & 1.69$\pm$ 0.06 & 138$\pm$ 1  \\ 
CU Cha & J & 20170406 & 58.2 & 32 & 1.42$\pm$ 0.12 & 117$\pm$ 3  \\ 
CU Cha & H & 20180413 & 58.2 & 36 & 1.5$\pm$ 0.12 & 112$\pm$ 2  \\ 
FU Ori & J & 20180103 & 58.2 & 24 & 0.16$\pm$ 0.03 & 87$\pm$ 6  \\ 
GW Ori & J & 20180104 & 58.2 & 32 & 0.48$\pm$ 0.1 & 96$\pm$ 6  \\ 
GW Ori & H & 20180104 & 58.2 & 36 & 0.34$\pm$ 0.11 & 110$\pm$ 10  \\ 
HD 100453 & J & 20150410 & 14.5 & 140 & 0.07$\pm$ 0.22 & 41$\pm$ 93  \\ 
HD 100546 & J & 20170220 & 43.6 & 40 & 1.16$\pm$ 0.07 & 60$\pm$ 2  \\ 
HD 101412 & H & 20180319 & 59.6 & 40 & 0.68$\pm$ 0.05 & 92$\pm$ 2  \\ 
HD 104237 & J & 20170407 & 58.2 & 32 & 0.44$\pm$ 0.05 & 98$\pm$ 3  \\ 
HD 104237 & J & 20180317 & 58.2 & 32 & 0.31$\pm$ 0.01 & 94$\pm$ 1  \\ 
HD 104237 & J & 20180520 & 58.2 & 32 & 0.38$\pm$ 0.04 & 119$\pm$ 3  \\ 
HD 104237 & J & 20190217 & 58.2 & 32 & 0.51$\pm$ 0.04 & 121$\pm$ 2  \\ 
HD 139614 & J & 20170406 & 58.2 & 64 & 0.46$\pm$ 0.09 & 179$\pm$ 5  \\ 
HD 139614 & H & 20180608 & 58.2 & 28 & 0.56$\pm$ 0.03 & 11$\pm$ 1  \\ 
HD 139614 & J & 20190513 & 58.2 & 36 & 0.17$\pm$ 0.08 & 130$\pm$ 14  \\ 
HD 141569 & J & 20180609 & 58.2 & 32 & 0.65$\pm$ 0.05 & 105$\pm$ 2  \\ 
HD 141569 & J & 20190223 & 58.2 & 32 & 0.52$\pm$ 0.06 & 114$\pm$ 3  \\ 
HD 142527 & H & 20140425 & 4.4 & 92 & 0.81$\pm$ 0.15 & 40$\pm$ 5  \\ 
HD 142666 & J & 20170703 & 58.2 & 20 & 0.49$\pm$ 0.06 & 84$\pm$ 4  \\ 
HD 142666 & J & 20180609 & 58.2 & 32 & 0.46$\pm$ 0.02 & 79$\pm$ 1  \\ 
HD 144432 & H & 20150709 & 58.2 & 32 & 1.26$\pm$ 0.09 & 175$\pm$ 2  \\ 
HD 145718 & J & 20180607 & 58.2 & 32 & 1.08$\pm$ 0.16 & 102$\pm$ 4  \\ 
HD 145718 & H & 20180608 & 58.2 & 32 & 1.51$\pm$ 0.18 & 82$\pm$ 3  \\ 
HD 158643 & J & 20180609 & 58.2 & 32 & 0.5$\pm$ 0.06 & 1$\pm$ 3  \\ 
HD 158643 & J & 20190223 & 58.2 & 32 & 0.55$\pm$ 0.02 & 3$\pm$ 1  \\ 
HD 169142 & J & 20140425 & 58.2 & 56 & 0.45$\pm$ 0.13 & 175$\pm$ 8  \\ 
HD 176386 & H & 20180607 & 58.2 & 32 & 0.28$\pm$ 0.02 & 2$\pm$ 2  \\ 
HD 176386 & H & 20180816 & 58.2 & 32 & 0.27$\pm$ 0.05 & 2$\pm$ 5  \\ 
HD 176386 & J & 20180817 & 58.2 & 64 & 0.15$\pm$ 0.14 & 40$\pm$ 27  \\ 
HD 34700 A & J & 20180103 & 58.2 & 32 & 0.65$\pm$ 0.13 & 102$\pm$ 6  \\ 
HD 34700 A & H & 20180103 & 58.2 & 32 & 0.36$\pm$ 0.05 & 104$\pm$ 4  \\ 
HD 36917 & J & 20171231 & 58.2 & 32 & 0.21$\pm$ 0.03 & 31$\pm$ 4  \\ 
HD 36917 & H & 20190126 & 58.2 & 36 & 0.79$\pm$ 0.03 & 44$\pm$ 1  \\ 
HD 37806 & J & 20171231 & 58.2 & 32 & 0.89$\pm$ 0.05 & 129$\pm$ 2  \\ 
HD 38087 & J & 20180103 & 58.2 & 32 & 1.3$\pm$ 0.06 & 109$\pm$ 1  \\ 
HD 45677 & J & 20171231 & 58.2 & 32 & 0.42$\pm$ 0.04 & 46$\pm$ 3  \\ 
HD 45677 & H & 20180101 & 58.2 & 32 & 0.46$\pm$ 0.04 & 11$\pm$ 3  \\ 
HD 50138 & J & 20180104 & 58.2 & 32 & 0.29$\pm$ 0.06 & 143$\pm$ 6  \\ 
HD 85567 & J & 20180103 & 58.2 & 32 & 0.45$\pm$ 0.05 & 71$\pm$ 3  \\ 
HD 85567 & J & 20180520 & 58.2 & 32 & 0.46$\pm$ 0.02 & 128$\pm$ 1  \\ 
HD 85567 & H & 20190127 & 58.2 & 28 & 0.48$\pm$ 0.03 & 84$\pm$ 2  \\ 
HD 95881 & J & 20180104 & 58.2 & 40 & 0.91$\pm$ 0.09 & 86$\pm$ 3  \\ 
HD 98800 & H & 20190127 & 34.9 & 28 & 0.74$\pm$ 0.1 & 154$\pm$ 4  \\ 
HD 98922 & J & 20180321 & 58.2 & 32 & 0.41$\pm$ 0.07 & 64$\pm$ 5  \\ 
Hen 3-1330 & J & 20190512 & 58.2 & 32 & 2.02$\pm$ 0.06 & 27$\pm$ 1  \\ 
Hen 3-225 & J & 20190127 & 58.2 & 32 & 0.47$\pm$ 0.05 & 147$\pm$ 3  \\ 
Hen 3-225 & H & 20190127 & 58.2 & 32 & 0.21$\pm$ 0.08 & 39$\pm$ 12  \\ 
Hen 3-365 & J & 20170406 & 58.2 & 32 & 0.79$\pm$ 0.09 & 166$\pm$ 3  \\ 
HR 5999 & J & 20170406 & 58.2 & 32 & 1.13$\pm$ 0.11 & 28$\pm$ 3  \\ 
HR 5999 & J & 20170702 & 58.2 & 36 & 0.32$\pm$ 0.19 & 19$\pm$ 17  \\ 
HT Lup & H & 20190514 & 52.4 & 64 & 0.77$\pm$ 0.12 & 36$\pm$ 4  \\ 
MWC 147 & J & 20171231 & 58.2 & 32 & 0.79$\pm$ 0.02 & 88$\pm$ 1  \\ 
MWC 147 & H & 20190127 & 58.2 & 32 & 1.0$\pm$ 0.07 & 97$\pm$ 2  \\ 
MWC 166 & J & 20170406 & 58.2 & 16 & 0.81$\pm$ 0.05 & 48$\pm$ 2  \\ 
MWC 275 & J & 20140424 & 58.2 & 32 & 0.8$\pm$ 0.34 & 34$\pm$ 12  \\ 
MWC 297 & H & 20180608 & 58.2 & 32 & 1.21$\pm$ 0.05 & 94$\pm$ 1  \\ 
MWC 297 & H & 20180817 & 43.6 & 32 & 1.15$\pm$ 0.04 & 99$\pm$ 1  \\ 
MWC 614 & J & 20180816 & 58.2 & 64 & 0.94$\pm$ 0.07 & 95$\pm$ 2  \\ 
MWC 614 & H & 20180816 & 58.2 & 64 & 1.24$\pm$ 0.11 & 101$\pm$ 2  \\ 
MWC 789 & H & 20181120 & 58.2 & 40 & 0.92$\pm$ 0.13 & 37$\pm$ 4  \\ 
MWC 863 & J & 20140424 & 58.2 & 32 & 2.95$\pm$ 0.28 & 56$\pm$ 3  \\ 
PDS 66 & J & 20160306 & 59.6 & 104 & 0.82$\pm$ 0.06 & 99$\pm$ 2  \\ 
Ty CrA & H & 20180608 & 58.2 & 32 & 0.33$\pm$ 0.04 & 148$\pm$ 3  \\ 
Ty CrA & H & 20180817 & 52.4 & 32 & 0.15$\pm$ 0.04 & 164$\pm$ 7  \\ 
V1295 Aql & H & 20180608 & 58.2 & 32 & 0.59$\pm$ 0.06 & 104$\pm$ 3  \\ 
V1295 Aql & J & 20180816 & 58.2 & 64 & 0.58$\pm$ 0.06 & 75$\pm$ 3  \\ 
V1295 Aql & H & 20180816 & 58.2 & 32 & 0.56$\pm$ 0.04 & 53$\pm$ 2  \\ 
V921 Sco & H & 20190513 & 58.2 & 32 & 0.98$\pm$ 0.21 & 138$\pm$ 6  \\ 
WRAY 15-535 & J & 20180319 & 58.2 & 32 & 2.1$\pm$ 0.09 & 53$\pm$ 1  \\ 
WRAY 15-535 & J & 20190222 & 58.2 & 32 & 2.02$\pm$ 0.1 & 58$\pm$ 1  \\ 
\enddata
\tablecomments{All epochs observed as part of the Gemini-LIGHTS survey. PA and \%Pol are the average polarization angle and \% polarization of stellar and instrumental polarization removed.}
\end{deluxetable*}

==> Gemini-LIGHTS_AAS_Submitted_Version_arxiv_submission copy/tables/target_properties.tex <==
\clearpage
%\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{lccccc}
\tablecaption{Gemini-LIGHTS Target Characteristics}
\tablehead{
\colhead{Target} & \colhead{Mass} & \colhead{Age} & \colhead{Teff} & \colhead{log$_{10}$(L)} & \colhead{Disk Classification} \\
\colhead{} & \colhead{(M\textsubscript{\(\odot\)})} & \colhead{(Myr)} & \colhead{(K)} & \colhead{log$_{10}$((L\textsubscript{\(\odot\)}))} & \colhead{} }
\label{tbl:target_properties}
\startdata
AK Sco & 1.4 $^{+0.07}_{-0.07}$ (b) & 8.38 $^{+1.72}_{-0.42}$ (b) & 6250 $^{+250}_{-250}$ (b) & 0.62 $^{+0.03}_{-0.01}$ (b) & Cont  \\ 
CU Cha & 2.25 $^{+0.11}_{-0.14}$ (b) & 4.37 $^{+1.11}_{-0.32}$ (b) & 10500 $^{+500}_{-500}$ (b) & 1.54 $^{+0.07}_{-0.06}$ (b) & Ring  \\ 
FU Ori & 0.3  (f) & 2.0   (i) & \nodata & \nodata & Irr  \\ 
GW Ori & 2.8   (ab) & 5.0   (j) & 5500.0   (ag) & 1.68 $^{+0.1}_{-0.08}$ (ah) & Irr  \\ 
HD 100453 & 1.25 $^{+0.06}_{-0.06}$ (b) & 6.53 $^{+0.45}_{-0.49}$ (b) & 7250 $^{+250}_{-250}$ (b) & 0.79 $^{+0.02}_{-0.0}$ (b) & Spiral, Cont  \\ 
HD 100546 & 2.06 $^{+0.1}_{-0.12}$ (b) & 5.48 $^{+1.41}_{-0.77}$ (b) & 9750 $^{+500}_{-500}$ (b) & 1.37 $^{+0.07}_{-0.05}$ (b) & Cont  \\ 
HD 101412 & 2.1 $^{+0.11}_{-0.11}$ (b) & 4.37 $^{+0.22}_{-0.32}$ (b) & 9750 $^{+250}_{-250}$ (b) & 1.58 $^{+0.05}_{-0.04}$ (b) & Nondet  \\ 
HD 104237 & 1.85 $^{+0.09}_{-0.09}$ (b) & 5.48 $^{+0.27}_{-0.4}$ (b) & 8000 $^{+250}_{-250}$ (b) & 1.33 $^{+0.04}_{-0.01}$ (b) & Undet  \\ 
HD 139614 & 1.48 $^{+0.07}_{-0.07}$ (b) & 14.49 $^{+1.41}_{-3.6}$ (b) & 7750 $^{+250}_{-250}$ (b) & 0.77 $^{+0.03}_{-0.01}$ (b) & Cont  \\ 
HD 141569 & 1.86 $^{+0.09}_{-0.09}$ (b) & 8.62 $^{+11.38}_{-1.19}$ (b) & 9750 $^{+250}_{-250}$ (b) & 1.22 $^{+0.03}_{-0.03}$ (b) & Ring  \\ 
HD 142527 & 1.61 $^{+0.12}_{-0.08}$ (b) & 6.63 $^{+0.33}_{-1.55}$ (b) & 6500 $^{+250}_{-250}$ (b) & 0.96 $^{+0.03}_{-0.0}$ (b) & Spiral, Ring  \\ 
HD 142666 & 1.49 $^{+0.08}_{-0.08}$ (b) & 9.33 $^{+0.77}_{-0.47}$ (b) & 7500 $^{+250}_{-250}$ (b) & 0.94 $^{+0.04}_{-0.05}$ (b) & Cont  \\ 
HD 144432 & 1.39 $^{+0.07}_{-0.07}$ (b) & 4.98 $^{+0.25}_{-0.55}$ (b) & 7500 $^{+250}_{-250}$ (b) & 0.97 $^{+0.04}_{-0.01}$ (b) & Nondet  \\ 
HD 145718 & 1.6 $^{+0.08}_{-0.08}$ (b) & 9.8 $^{+2.8}_{-0.49}$ (b) & 8000 $^{+250}_{-250}$ (b) & 0.9 $^{+0.05}_{-0.04}$ (b) & Cont  \\ 
HD 158643 & 3.35 $^{+0.79}_{-0.22}$ (b) & 1.22 $^{+0.29}_{-0.57}$ (b) & 9800 $^{+900}_{-300}$ (b) & 2.22 $^{+0.26}_{-0.07}$ (b) & Nondet  \\ 
HD 169142 & 2.0 $^{+0.13}_{-0.13}$ (b) & 8.98 $^{+11.02}_{-3.9}$ (b) & 10700 $^{+800}_{-900}$ (b) & 1.31 $^{+0.12}_{-0.22}$ (b) & Ring  \\ 
HD 176386 & 2.3 $^{+0.14}_{-0.3}$ (b) & 4.05 $^{+15.95}_{-0.57}$ (b) & 10700 $^{+800}_{-900}$ (b) & 1.58 $^{+0.12}_{-0.22}$ (b) & Nondet  \\ 
HD 34700 A & 2.66 $^{+0.32}_{-0.13}$ (b) & 1.4 $^{+0.23}_{-0.44}$ (b) & 5900 $^{+110}_{-100}$ (b) & 1.36 $^{+0.1}_{-0.02}$ (b) & Spiral, Ring  \\ 
HD 36917 & 3.71 $^{+0.94}_{-0.75}$ (b) & 0.99 $^{+0.9}_{-0.5}$ (b) & 11215 $^{+1109}_{-1316}$ (b) & 2.43 $^{+0.24}_{-0.29}$ (b) & Nondet  \\ 
HD 37806 & 3.11 $^{+0.55}_{-0.33}$ (b) & 1.56 $^{+0.64}_{-0.6}$ (b) & 10475 $^{+1025}_{-675}$ (b) & 2.17 $^{+0.19}_{-0.14}$ (b) & Undet  \\ 
HD 38087 & 3.21 $^{+0.79}_{-0.38}$ (b) & 1.75 $^{+9.15}_{-0.64}$ (b) & 13600 $^{+2900}_{-830}$ (b) & 2.19 $^{+0.3}_{-0.22}$ (b) & Nondet  \\ 
HD 45677 & 4.72 $^{+1.19}_{-0.39}$ (b) & 0.61 $^{+3.77}_{-0.3}$ (b) & 16500 $^{+3000}_{-750}$ (b) & 2.88 $^{+0.32}_{-0.17}$ (b) & Cont  \\ 
HD 50138 & 4.17 $^{+0.46}_{-0.33}$ (b) & 0.63 $^{+0.19}_{-0.18}$ (b) & 9450 $^{+450}_{-450}$ (b) & 2.46 $^{+0.13}_{-0.09}$ (b) & Cont  \\ 
HD 85567 & 6.32 $^{+0.53}_{-0.39}$ (b) & 0.22 $^{+0.05}_{-0.05}$ (b) & 13000 $^{+500}_{-500}$ (b) & 3.19 $^{+0.1}_{-0.08}$ (b) & Undet  \\ 
HD 95881 & 5.5 $^{+0.5}_{-0.28}$ (b) & 0.28 $^{+0.05}_{-0.07}$ (b) & 10000 $^{+250}_{-250}$ (b) & 2.85 $^{+0.1}_{-0.07}$ (b) & Undet  \\ 
HD 98800 & 0.7   (ab) & 8.5 $^{+1.5}_{-1.5}$ (h) & 4200   (al) & 0.33   (al) & Undet  \\ 
HD 98922 & 6.17 $^{+0.37}_{-0.31}$ (b) & 0.2 $^{+0.01}_{-0.04}$ (b) & 10500 $^{+250}_{-250}$ (b) & 3.03 $^{+0.06}_{-0.05}$ (b) & Undet  \\ 
Hen 3-1330 & 9.0  &  \nodata &    22280   (ai) & 5.3   (ai) & Nondet  \\ 
Hen 3-225 & 7.46 $^{+0.51}_{-0.37}$ (b) & 0.17 $^{+0.02}_{-0.03}$ (b) & 19000 $^{+500}_{-500}$ (b) & 3.55 $^{+0.09}_{-0.07}$ (b) & Nondet  \\ 
Hen 3-365 & 17.72 $^{+10.87}_{-6.72}$ (b) & 0.02 $^{+0.05}_{-0.01}$ (b) & 19500 $^{+5000}_{-3000}$ (b) & 4.6 $^{+0.64}_{-0.53}$ (b) & Irr  \\ 
HR 5999 & 2.43 $^{+0.12}_{-0.12}$ (b) & 2.73 $^{+0.26}_{-0.35}$ (b) & 8500 $^{+250}_{-250}$ (b) & 1.72 $^{+0.05}_{-0.04}$ (b) & Nondet  \\ 
HT Lup & 1.3 $^{+0.2}_{-0.2}$ (d) & 0.5 $^{+0.02}_{-0.4}$ (d) & 4247 $^{+161}_{-237}$ (k) & 0.51 $^{+0.01}_{-0.01}$ (k) & Ring  \\ 
MWC 147 & 5.16 $^{+1.84}_{-1.29}$ (b) & 0.42 $^{+0.53}_{-0.28}$ (b) & 14000 $^{+2125}_{-2900}$ (b) & 2.97 $^{+0.27}_{-0.4}$ (b) & Nondet  \\ 
MWC 166 & 12.3 $^{+4.2}_{-4.2}$ (e) & 0.08 $^{+0.08}_{-0.08}$ (e) & 29500 $^{+1000}_{-1000}$ (e) & 4.11 $^{+0.37}_{-0.37}$ (e) & Nondet  \\ 
MWC 275 & 1.83 $^{+0.09}_{-0.09}$ (b) & 7.6 $^{+1.05}_{-1.22}$ (b) & 9250 $^{+250}_{-250}$ (b) & 1.2 $^{+0.06}_{-0.03}$ (b) & Ring  \\ 
MWC 297 & 16.9 $^{+1.87}_{-1.22}$ (b) & 0.03 $^{+0.01}_{-0.01}$ (b) & 24500 $^{+1500}_{-1500}$ (b) & 4.59 $^{+0.12}_{-0.12}$ (b) & Cont  \\ 
MWC 614 & 2.98 $^{+0.18}_{-0.3}$ (b) & 1.66 $^{+0.54}_{-0.26}$ (b) & 9500 $^{+200}_{-200}$ (b) & 2.05 $^{+0.09}_{-0.14}$ (b) & Cont  \\ 
MWC 789 & 2.6 $^{+0.3}_{-0.14}$ (b) & 2.56 $^{+0.43}_{-0.67}$ (b) & 11000 $^{+500}_{-500}$ (b) & 1.94 $^{+0.17}_{-0.12}$ (b) & Irr  \\ 
MWC 863 & 1.89 $^{+0.1}_{-0.1}$ (b) & 5.48 $^{+0.44}_{-0.27}$ (b) & 9000 $^{+250}_{-250}$ (b) & 1.37 $^{+0.04}_{-0.04}$ (b) & Undet  \\ 
PDS 66 & 1.2   (ak) & 6.0 $^{+1.0}_{-1.0}$ (g) & 5035 $^{+19}_{-19}$ (ak) & 0.0 $^{+0.01}_{-0.01}$ (ak) & Ring  \\ 
Ty CrA & 2.06 $^{+0.22}_{-0.19}$ (b) & 6.38 $^{+13.62}_{-2.01}$ (b) & 10700 $^{+800}_{-900}$ (b) & 1.41 $^{+0.14}_{-0.23}$ (b) & Nondet  \\ 
V1295 Aql & 5.89 $^{+0.8}_{-0.76}$ (b) & 0.22 $^{+0.11}_{-0.07}$ (b) & 9500 $^{+200}_{-200}$ (b) & 2.9 $^{+0.16}_{-0.2}$ (b) & Nondet  \\ 
V921 Sco & 19.96 $^{+6.98}_{-5.0}$ (b) & 0.02 $^{+0.03}_{-0.01}$ (b) & 29000 $^{+3882}_{-4500}$ (b) & 4.76 $^{+0.33}_{-0.34}$ (b) & Undet  \\ 
WRAY 15-535 & 17.5 $^{+2.5}_{-2.5}$ (c) & \nodata &    20000 $^{+3000}_{-3000}$ (aj) & 6.0   (aj) & Undet  \\ 
\enddata
\tablecomments{Stellar and disk characteristics of stellar mass, Age, Teff, Luminosity, and our disk classification. Disk classification described in section \ref{sec:catagories}. In the table Undet is short for Undetermined and Nondet is short for Non-detections. Citations for specific values are from the following: (b) \citet{Vioque2018}, (c) \citet{Maravelias2018}, (d) \citet{Garufi2020}, (e) \citet{Fairlamb2015}, (f) \citet{Zhu2007}, (g) \citet{Murphy2013}, (h) \citet{2018Ribas}, (i)\citet{Beck2012}, (j) \citet{Monnier2019}, (k) \citet{Gaia2018}, (l) \citet{Takami2018}}
\end{deluxetable*}
%\end{longrotatetable}
